Geometric Approaches to Matrix Normalization and Graph Balancing

Normal matrices, or matrices which commute with their adjoints, are of fundamental importance in pure and applied mathematics. In this paper, we study a natural functional on the space of square complex matrices whose global minimizers are normal matrices. We show that this functional, which we refer to as the non-normal energy, has incredibly well-behaved gradient descent dynamics: despite it being non-convex, we show that the only critical points of the non-normal energy are the normal matrices, and that its gradient descent trajectories fix matrix spectra and preserve the subset of real matrices. We also show that, even when restricted to the subset of unit Frobenius norm matrices, the gradient flow of the non-normal energy retains many of these useful properties. This is applied to prove that low-dimensional homotopy groups of spaces of unit norm normal matrices vanish; for example, we show that the space of $d \times d$ complex unit norm normal matrices is simply connected for all $d \geq 2$. Finally, we consider the related problem of balancing a weighted directed graph -- that is, readjusting its edge weights so that the weighted in-degree and out-degree is the same at each node. We adapt the non-normal energy to define another natural functional whose global minima are balanced graphs and show that gradient descent of this functional always converges to a balanced graph, while preserving graph spectra and realness of the weights. Our results were inspired by concepts from symplectic geometry and Geometric Invariant Theory, but we mostly avoid invoking this machinery and our proofs are generally self-contained.

==> extrastuff.tex <==
% \begin{remark}
% 	Our work in this paper is heavily inspired by Mumford's \emph{Geometric Invariant Theory (GIT)}~\cite{mumford_geometric_1994} (see~\cite{thomas_notes_2005} for a nice introduction) and Kirwan's work relating GIT and symplectic geometry~\cite{kirwan_cohomology_1984}. One of our goals was to make our arguments---especially the fundamentally elementary ones---as accessible as possible, so we have mostly avoided explicitly invoking GIT in what follows, but it was very much on our minds as we were working on this paper.
% \end{remark}


% \footnote{A critic might object that all of our results are in some sense implicit in work of Mumford, Kirwan, Ness, and others. While there is some validity to this objection, these tools do not seem to be well known in the matrix and graph optimization communities, so there is value in working the theory out in that context. \tom{I see the point of this comment, but it maybe sounds a bit pessimistic currently...}}


% \section{The Space of Normal Matrices}

% This section considers the basic geometric and topological structure of the space $\normal$ of normal $d\times d$ matrices. We use basic terminology from the field of symplectic geometry. In our previous papers, we give short and elementary overviews of the necessary concepts from symplectic geometry, with a view toward understanding similar spaces of structured matrices (e.g., spaces consisting of unit norm, tight frames). As such, we only give short reminders regarding the meaning of any symplectic terminology in this section, and  we refer the reader to~\cite[Section 2]{needham2021symplectic} and~\cite[Section 2.1]{needham2022toric} for more in-depth exposition. For a general reference on symplectic geometry, we recommend \cite{da2001lectures}.

% \subsection{Normal Matrices as a Real Algebraic Variety}

% We begin with a brief recollection of some results on the structure of $\normal$ coming from the perspective of real algebraic geometry. If we write the entries of a matrix $A \in \C^{d \times d}$ as  $A = (a_{ij})_{i,j = 1}^d$, then $A \in \normal$ if and only if
% \[
% \sum_{k=1}^d a_{ik}\overline{a_{jk}} - \overline{a_{ki}}a_{kj}  = 0
% \]
% holds for all $i,j = 1,\ldots, d$. Each of these equations defines the zero set of a quadratic polynomial in the real and imaginary coordinates of the entries of $A$. Since the polynomials involve conjugation, we conclude that $\normal$ is a real algebraic subvariety of $\Cd \approx \R^{2d \times 2d}$, but not a complex one. The real algebraic geomery of $\normal$ has been thoroughly studied. The following summarizes results from \cite{ikramov1998dimension} and \cite{friedland2002normal}.

% \begin{thm}[\!\cite{ikramov1998dimension,friedland2002normal}]\label{thm:prior_results}
% \begin{enumerate}
%     \item The space of normal matrices $\normal$ is an irreducible homogeneous algebraic variety of dimension $d(d+1)$.
%     \item The set of smooth points of $\normal$ consists of all normal matrices with pairwise distinct eigenvalues.
%     \item The set of smooth points in $\normal$ is connected.
% \end{enumerate}
% \end{thm}

% Similar results were obtained for the space of conjugate normal matrices in \cite{ghasemi2008dimension}.



% \subsection{Normal Matrices and Symplectic Geometry}\label{sec:symplectic}

% We consider $\C^{d \times d}$ as an inner product space, endowed with the Frobenius inner product: for $A,B \in \Cd$, 
% \[
% \langle A, B \rangle = \mathrm{Tr} \big(B^\ast A \big),
% \]
% where $B^\ast$ denotes the conjugate transpose of $B$. The negative imaginary part defines the standard symplectic structure $\omega$ on $\Cd$, that is, 
% \[
% \omega_A(S,T) = -\mathrm{Im} \langle S, T \rangle,
% \]
% where $A \in \Cd$ and $S,T \in T_A \Cd \approx \Cd$. 


% Consider the action of $\SU(d)$ on $\Cd$ by conjugation,
% \[
% U \cdot A = UAU^\ast.
% \]
% In what follows, we use $\mathfrak{su}(d)$ to denote the Lie algebra of $\SU(d)$; namely, $\mathfrak{su}(d)$ is the space of traceless skew-Hermitian matrices. We use $\mathfrak{su}(d)^\ast$ to denote the dual space. The following result shows that this action is \emph{Hamiltonian}---see \cite[Section 2.1]{needham2022toric} for relevant definitions.

% % We recall that the \emph{adjoint action} of a matrix Lie group $G$ on its Lie algebra $\mathfrak{g}$ is the action defined by
% % \[
% % G \times \mathfrak{g} \ni (A,X) \mapsto \mathrm{Ad}_A(X):= AXA^\ast \in \mathfrak{g}.
% % \]
% % Then the \emph{coadjoint action} of $G$ on $\mathfrak{g}^\ast$ is defined by
% % \[
% % G \times \mathfrak{g}^\ast \ni (A,\xi) \mapsto \mathrm{Ad}^\ast_A(\xi) \in \mathfrak{g}^\ast, \quad \mbox{where} \quad \mathrm{Ad}^\ast_A(\xi)(X) := \xi(\mathrm{Ad}_{A^{-1}}(X)).
% % \]

% % Consider the map $\mu_d:\Cd \to \mathfrak{su}(d)^\ast$ defined by
% % \begin{equation}\label{eqn:SUd_momentum_map}
% %     \mu_d(A)(X) = \frac{i}{2} \mathrm{Tr}\left(X\big(AA^\ast - A^\ast A\big)\right).
% % \end{equation}

% \begin{prop}\label{prop:momentum_map}
%     The conjugation action of $\SU(d)$ on $\Cd$ is Hamiltonian, with momentum map $\mu_d:\Cd \to \mathfrak{su}(d)^\ast$ defined by
%     \[
%     \mu_d(A)(X) = \frac{i}{2} \mathrm{Tr}\left(X\big(AA^\ast - A^\ast A\big)\right)
%     \]
%     for $A \in \Cd$ and $X \in \mathfrak{su}(d)$. 
% \end{prop}

% \begin{proof}
%     Let us first show that $\mu_d$ is $\operatorname{Ad}^\ast$-equivariant. We have, for $A \in \Cd$, $U \in \SU(d)$ and $X \in \mathfrak{su}(d)$,
%     \begin{align*}
%     \mu_d(U \cdot A)(X) &= \mu_d(UAU^\ast)(X) \\
%     &= \frac{i}{2} \operatorname{Tr} \left(X \big((UAU^\ast)(UAU^\ast)^\ast - (UAU^\ast)^\ast (UAU^\ast)\big) \right) = \frac{i}{2} \operatorname{Tr}\left(X \big(UAA^\ast U^\ast - U A^\ast A U^\ast \big) \right) \\
%     &= \frac{i}{2} \operatorname{Tr}\left(X U \big(AA^\ast  -  A^\ast A  \big)U^\ast \right) = \frac{i}{2} \operatorname{Tr} \left((U^\ast X U) (AA^\ast - A^\ast A) \right)
%     \\
%     &= \mu_d(A)(U^\ast X U) = \mu_d(A)\big(\!\operatorname{Ad}_{U^\ast}(X)\big) = \operatorname{Ad}^\ast_U(\mu(A))(X).
%     \end{align*}

%     Next, we check that, for $A \in \Cd$, $S \in T_A \Cd \approx \Cd$ and $X \in \mathfrak{su}(d)$, 
%     \begin{equation}\label{eqn:momentum_equation_normal}
%         D_A \mu_d(S)(X) = \omega_A(X_A, S),
%     \end{equation}
%     where $X_A$ is the infinitesimal vector field associated to $X$, evaluated at $A$. We have
%     \begin{align*}
%         D_A \mu_d(S)(X) &= \left. \frac{d}{d\epsilon} \right|_{\epsilon = 0} \mu_d(A + \epsilon S)(X) \\
%         &= \left. \frac{d}{d\epsilon} \right|_{\epsilon = 0} \frac{i}{2} \operatorname{Tr} \left(X \big((A + \epsilon S)(A + \epsilon S)^\ast - (A + \epsilon S)^\ast (A + \epsilon S) \big) \right) \\
%         &= \frac{i}{2} \operatorname{Tr} \left(X \big(AS^\ast + SA^\ast - A^\ast S - S^\ast A \big) \right).
%     \end{align*}
%     Next, observe that the infinitesimal vector field is given by
%     \[
%     X_A = \left. \frac{d}{d\epsilon}\right|_{\epsilon = 0} \exp(\epsilon X) \cdot A = \left. \frac{d}{d\epsilon}\right|_{\epsilon = 0} \exp(\epsilon X)  A\mathrm{exp}(\epsilon X)^\ast = XA + A X^\ast = XA - A X.
%     \]
%     It follows that
%     \begin{align*}
%         \omega_A(X_A,S) &= - \operatorname{Im} \operatorname{Tr} \left(S^\ast \big(XA - AX) \right) \\
%         &= \frac{i}{2} \operatorname{Tr} \left(S^\ast X A - S^\ast A X - A^\ast X^\ast S + X^\ast A^\ast S \right) \\
%         &= \frac{i}{2} \operatorname{Tr} \left(X \big(AS^\ast + SA^\ast - A^\ast S - S^\ast A \big) \right),
%     \end{align*}
%     where we have used cyclic permutation invariance of trace and the fact that $X$ is skew-Hermitian. Putting all of this together establishes \eqref{eqn:momentum_equation_normal}.
% \end{proof}

% It will be convenient to identify $\mathfrak{su}(d)^\ast$ with the space $\mathscr{H}_0(d)$ of $d \times d$ traceless Hermitian matrices via the isomorphism
% \begin{align*}
%     \mathscr{H}_0(d) &\to \mathfrak{su}(d)^\ast \\
%     Y &\mapsto \big(X \mapsto \frac{i}{2}\mathrm{Tr}(XY)\big).
% \end{align*}
% Under this identification, we can express the momentum map (via a slight abuse of notation) as follows. We use $[\cdot, \cdot]$ to denote the standard commutator defined by $[X,Y]=XY-YX$.

% \begin{cor}\label{cor:ud_momentum_hermitian}
%     Under the identification $\mathfrak{su}(d)^\ast \approx \mathscr{H}_0(d)$ given above, the momentum map $\mu_d$ for the $\unitary(d)$-action is expressed as 
%     \[
%     \mu_d(A) = [A,A^\ast].
%     \]
% \end{cor}



% We can also act on $\Cd$ by scalar multiplication. More precisely, consider the action of $\unitary(1)$ on $\Cd$ by
% \[
% 	e^{i\theta} \cdot A = e^{i\theta}A.
% \]
% This action is also Hamiltonian, as we demonstrate below. Here, we identify $\mathfrak{u}(1)^\ast \approx \R$ in the obvious way.

% \begin{prop}\label{prop:scalar multiplication}
%     The scalar action of $\unitary(1)$ on $\Cd$ is Hamiltonian, with momentum map $\nu: \Cd \to \R$ given by ${\nu(A) := - \frac{1}{2}(\|A\|^2-1)}$.
% \end{prop}

% \begin{proof}
% 	Since $\nu(e^{i\theta} A) = \|A\|^2 =  \nu(A)$, the action of $\unitary(1)$ preserves level sets of $\nu$. Moreover, the Hamiltonian vector field $X$ associated to the $\unitary(1)$-action is given by
% 	\[
% 		Y_A = \left. \frac{d}{dt} \right|_{t=0} e^{it}A = iA,
% 	\]
% 	so
% 	\[
% 		\omega_A(Y_A,S) = -\operatorname{Im} \operatorname{Tr}(S^\ast i A) = -\operatorname{Re}\operatorname{Tr}(S^\ast A) = -\frac{1}{2} \operatorname{Tr}(S^\ast A + A^\ast S) = \left. \frac{d}{d\epsilon}\right|_{\epsilon=0} -\frac{1}{2}(\|A + \epsilon S \|^2-1) = (d\nu)_A(S),
% 	\]
% 	and hence $\nu(A) = - \frac{1}{2}(\|A\|^2-1)$ is a momentum map for the $\unitary(1)$ action.
% \end{proof}

% \begin{remark}
% 	We have subtracted 1 in the definition of $\nu$ in order to ensure that the matrices of norm 1 are the inverse image of 0. This is purely for convenience to make the proof of \Cref{thm:connected} simpler; we could of course have defined $\nu$ by $A \mapsto -\frac{1}{2}(\|A\|^2-s)$ for any $s \in \R$, including $s=0$.
% \end{remark}

% Since the product of Hamiltonian actions is Hamiltonian, with momentum map given by the product of the individual momentum maps, \Cref{cor:ud_momentum_hermitian} and \Cref{prop:scalar multiplication} immediately imply:

% \begin{cor}\label{cor:product moment}
% 	The product action of  $\SU(d) \times \unitary(1)$ on $\Cd$ is Hamiltonian, with momentum map $\mu: \Cd \to \mathscr{H}_0(d) \times \R$ defined by
% 	\[
% 		\mu(A) = (\mu_d(A),\nu(A))= \left([A,A^\ast], -\frac{1}{2}(\|A\|^2-1)\right).
% 	\]
% \end{cor}


% \subsection{Connectedness of Unit Norm Normal Matrices}\label{sec:connectedness_unit_norm}

% Normality of matrices is scale-invariant, so the space of normal matrices is a cone, and hence obviously connected. More precisely, if we let $\mathcal{U}_d := \{A \in \Cd : \|A\|=1\}$ be the space of $d \times d$ matrices of Frobenius norm 1 and let $\unitnormal = \normal \cap \mathcal{U}_d$, then $\normal$ is a cone over $\unitnormal$. By \Cref{cor:product moment}, 
% \begin{equation}\label{eq:inverse image}
% 	\unitnormal = \mu^{-1}(0,0).
% \end{equation}

% We recall a theorem of Kirwan:

% \begin{thm}[{Kirwan~\cite[(9.1)]{kirwan_cohomology_1984} and~\cite[(3.1)]{kirwan_convexity_1984}; see also~\cite[Remark~5.8]{sjamaar_stratified_1991}}]\label{thm:level sets}
% 	Let $G$ be a compact group with a Hamiltonian action on the symplectic manifold $(M,\omega)$. If the momentum map $\Phi: M \to \mathfrak{g}^\ast$ is proper, then $\Phi^{-1}(0)$ is connected.
% \end{thm}

% Combining \Cref{thm:level sets} with \eqref{eq:inverse image}, we see that the space of normal matrices is a cone over a connected space:

% \begin{thm}\label{thm:connected}
% 	The space $\unitnormal$ of normal matrices with Frobenius norm 1 is connected.
% \end{thm}

% \begin{remark}	Friedland~\cite{friedland2002normal} argues that $\unitnormal$ is irreducible and the quasi-variety of its smooth points is connected. However, this is not quite enough to imply \Cref{thm:connected}, since irreducible real varieties can have connected components consisting entirely of non-smooth points (see, e.g., \cite[Figure~2]{cahill_connectivity_2017}).
% \end{remark}

% In fact, we will significantly generalize \Cref{thm:connected} below. We show in \Cref{thm:topology_unit_normal} that many higher homotopy groups of $\unitnormal$ vanish; in particular, $\unitnormal$ is always simply connected. This result will rely on the geometric and optimization theoretic techniques that we develop in the following section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% \begin{lem}\label{lem:no_spurious_local_mins}
% Consider the following commutative diagram of topological spaces and continuous maps
%     % https://q.uiver.app/#q=WzAsNCxbMCwwLCJYIl0sWzEsMCwiWSJdLFsyLDAsIlxcbWF0aGJie1J9Il0sWzEsMSwiWiJdLFswLDEsImciXSxbMSwyLCJmIl0sWzAsMywiXFx0aWxkZXtnfSIsMl0sWzMsMiwiXFx0aWxkZXtmfSIsMl0sWzEsMywiXFxwaSIsMl1d
% \[\begin{tikzcd}
% 	X & Y & {\mathbb{R}} \\
% 	& Z
% 	\arrow["g", from=1-1, to=1-2]
% 	\arrow["f", from=1-2, to=1-3]
% 	\arrow["{\tilde{g}}"', from=1-1, to=2-2]
% 	\arrow["{\tilde{f}}"', from=2-2, to=1-3]
% 	\arrow["\pi"', from=1-2, to=2-2]
% \end{tikzcd}\]
% Suppose that $Y$ is a convex subset of a real topological vector space, that $\tilde{g}$ is an open map and that $f$ is a convex function. Then $f \circ g$ has no spurious local minima.
% \end{lem}
%
% \tom{Notation used in the proof needs to be reconciled with the above (e.g., $U$ is a unitary matrix above, but an open subset in the proof).}
% \begin{proof}
%     Let $x_0$ be a local minimum of $f \circ g$. We will show that $x_0$ is a global minimum.
%
%     Consider $z_0 := \tilde{g}(x_0) = \pi \circ g(x_0)$. Let $U$ be an open neighborhood of $x_0$ such that $f \circ g(x) \geq f \circ g(x_0)$ for all $x \in U$. Then $W := \tilde{g}(U)$ is an open neighborhood of $z_0$ and for all $z = \tilde{g}(x) \in W$,
%     \[
%     \tilde{f}(z) = \tilde{f} \circ \tilde{g}(x) = f \circ g (x) \geq f\circ g(x_0) = \tilde{f} \circ \tilde{g} (x_0) = \tilde{f}(z_0),
%     \]
%     so that $z_0$ is a local minimum of $\tilde{f}$.
%
%     Now consider $V := \pi^{-1}(W)$. Since $\tilde{g}(x_0) = \pi \circ g (x_0)$, $V$ is an open neighborhood of $y_0 := g(x_0)$. Also, $\pi(y_0) = \pi \circ g (x_0) = \tilde{g}(x_0) = z_0$. For any $y \in V$,
%     \[
%     f(y) = \tilde{f} \circ \pi(y) \geq \tilde{f}(z_0) = \tilde{f} \circ \pi (y_0) = f(y_0),
%     \]
%     so that $y_0$ is a local minimum of $f$. By convexity of $f$ and $Y$, $y_0$ must be a global minimum of $f$. In particular, for any $g(x) \in Y$, $f \circ g(x) \geq f \circ g(x_0)$, so that $x_0$ is a global minimum of $f \circ g$.
% \end{proof}
%
%
% \begin{thm}
%     Let $(M,\omega)$ be a sympectic manifold. Let $G$ be a Lie group with a Hamiltonian action on $M$ with momentum map $\mu:M \to \mathfrak{g}^\ast$. For any convex and $\operatorname{Ad}^\ast$-invariant function $f:\mathfrak{g}^\ast \to \R$, the function $f \circ \mu:M \to \R$ has no spurious local minima.
% \end{thm}
%
% \begin{proof}
%     Consider the diagram
%     % https://q.uiver.app/#q=WzAsNCxbMCwwLCJNIl0sWzEsMCwiXFxtYXRoZnJha3tnfV5cXGFzdCJdLFsyLDAsIlxcbWF0aGJie1J9Il0sWzEsMSwiXFxtYXRoZnJha3tnfV5cXGFzdC9HIl0sWzAsMSwiZyJdLFsxLDIsImYiXSxbMCwzLCJcXHRpbGRle2d9IiwyXSxbMywyLCJcXHRpbGRle2Z9IiwyXSxbMSwzLCJcXHBpIiwyXV0=
% \[\begin{tikzcd}
% 	M & {\mathfrak{g}^\ast} & {\mathbb{R}} \\
% 	& {\mathfrak{g}^\ast/G}
% 	\arrow["\mu", from=1-1, to=1-2]
% 	\arrow["f", from=1-2, to=1-3]
% 	\arrow["{\tilde{\mu}}"', from=1-1, to=2-2]
% 	\arrow["{\tilde{f}}"', from=2-2, to=1-3]
% 	\arrow["\pi"', from=1-2, to=2-2]
% \end{tikzcd}\]
%     where $G$ acts on $\mathfrak{g}^\ast$ by the $\operatorname{Ad}^\ast$-action, $\pi$ is the quotient map $\tilde{g}:= \pi \circ g$, and $\tilde{f}$ is well-defined by the assumption of $\operatorname{Ad}^\ast$-invariance of $f$. By \cite[Theorem 3.19]{birtea2009openness}, $\tilde{g}$ is an open map. The result then follows from Lemma \ref{lem:no_spurious_local_mins}.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{cor}
%     Any local minimum of the non-normal energy $\energy$ is a normal matrix.
% \end{cor}

% \clay{Thoughts on gradient descent:}
%
% If we do gradient descent on $\energy$, the usual GIT theory should imply that we stay within the $\SL_d(\C)$-orbit of the starting point. In particular, for any non-nilpotent (assuming this really is the semi-stability condition) starting matrix $A$, this will imply that there is some $g \in \SL_d(\C)$ so that $g A g^{-1}$ is normal. My initial inclination is to try to do some sort of Hamilton--Moitra~\cite{hamilton_paulsen_2018} thing to get a bound just from knowledge of the existence of such a $g$. I guess the hypothesis would be that the Henrici departure from normality $\|A\|^2 - \sum |\lambda_i|^2 < \epsilon$, but I don't really see how to connect this to the Hamilton--Moitra approach. Note that in principle one can find $g$ by minimizing a Kempf--Ness function over $\SL_d(\C)/\SU(d) \simeq \R^{d^2-1}$, and this function is geodesically convex with respect to a natural hyperbolic metric on $\R^{d^2-1}$.
%
% Also, gradient descent will preserve realness, so if $A$ is real, there will be $g \in \SL_d(\C)$ so that $gA g^{-1}$ is real and normal. I presume this is enough to conclude that $g$ is also real: it certainly is enough if $A$ is, say, diagonalizable, because then the real span of the (real) eigenvectors of $g$ will be all of $\R^d$ and $g$ will have to preserve all of $\R^d$, and hence must be real.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{align}
% \frac{1}{2} D_A \energy (B) &=   \langle AA^\ast - A^\ast A, AB^\ast + BA^\ast - A^\ast B - B^\ast A \rangle \nonumber \\
% &= \langle A^\ast A A^\ast - A^\ast A^\ast A, B^\ast\rangle + \langle AA^\ast A - A^\ast A A, B\rangle - \langle AAA^\ast - AA^\ast A, B \rangle - \langle AA^\ast A^\ast - A^\ast A A^\ast, B^\ast \rangle \label{eqn:grad_calculation} \\
% &= -\left(\langle AAA^\ast - AA^\ast A - AA^\ast + A^\ast A A, B \rangle + \langle (AAA^\ast - AA^\ast A - AA^\ast + A^\ast A A)^\ast, B^\ast \rangle \right) \nonumber \\
% &= -2 \mathrm{Re} \langle AAA^\ast - AA^\ast A - AA^\ast + A^\ast A A, B \rangle \nonumber \\
% &= -2 \mathrm{Re} \langle [A,[A,A^\ast]], B \rangle, \nonumber
% \end{align}
% where \eqref{eqn:grad_calculation} follows by bilinearity of the inner product and properties of the conjugate transpose, so that
% \[
% D_A \energy (B) = \mathrm{Re} \langle -4 [A,[A,A^\ast]], B \rangle,
% \]
% and the claim follows.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \[
    % \left[
    % \begin{array}{ccccc}
    % 0&a_{11}&a_{12}& \cdots & a_{1(d-1)} \\
    % 0& a_{21} & a_{22} & \cdots & a_{2(d-1)} \\
    % \vdots&\vdots&\vdots&\vdots&\vdots \\
    % 0&a_{(d-1)1}&a_{(d-1)2}& \cdots & a_{(d-1)(d-1)} \\
    % 0&a_{d1}&a_{d2}& \cdots & a_{d(d-1)} 
    % \end{array}\right] = 
    % \left[
    % \begin{array}{ccccc}
    % a_{21}&a_{22}&a_{23}&\cdots & a_{2d} \\
    % a_{31}&a_{32}&a_{33}&\cdots & a_{3d} \\
    % \vdots&\vdots&\vdots&\vdots&\vdots \\
    % a_{d1}&a_{d2}&a_{d3}&\cdots & a_{dd} \\
    % 0&0&0&0&0 
    % \end{array}\right].
    % \]
    % We then count the independent constraints:
    % \begin{enumerate}
    %     \item The column and row of zeroes produce constraints
    %     \begin{align*}
    %         a_{21} &= a_{31} = \cdots = a_{d1} = 0, \mbox{ and}\\
    %         a_{d1} &= a_{d2} = \cdots = a_{d(d-1)} = 0,
    %     \end{align*}
    %     respectively. Exactly one of these is redudant ($a_{d1} = 0$), so this gives $2d-3$ constraints, overall.
    %     \item Now consider the submatrices obtained by deleting the first column and last row of these matrices. 
    %     \begin{enumerate}
    %         \item The upper triangles of these submatrices, including diagonals, produce $d(d-1)/2$ independent constraints of the form $a_{ij} = a_{(i+1)(j+1)}$.
    %         \item The remaining entries of these submatrices---the lower triangles, excluding diagonals---also produce constraints of the form $a_{ij} = a_{(i+1)(j+1)}$, but some of these are redundant. Indeed, those constraints of the form $a_{(d-1)j} = a_{d(j+1)}$ are implied by others that have already been counted: for $j=1$, $a_{(d-1)1}$ and $a_{d2}$ are already both known to be zero by point 1 above; for $j>1$, $a_{(d-1)j} = 0$ by point 2(a) (as $0 = a_{(d-2)(j-1)} = a_{(d-1)j}$) and $a_{d(j+1)} = 0$ by point 1. The total number of independent constraints is then equal to
    %         \[
    %         \frac{(d-2)(d-1)}{2} - (d-2)
    %         \]
    %         (the number of points in the lower triangle of the submatrix, minus the number of redundant constraints). 
    %     \end{enumerate}
    % \end{enumerate}
    % Putting this together, the total number of independent constraints is 
    % \[
    % 2d-3 + \frac{d(d-1)}{2} + \frac{(d-2)(d-1)}{2} - (d-2) = d^2-d.
    % \]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Jotting down some thoughts from text messages: think about the map $\delta: \Cd \to \R^d$ which records the diagonal of $[A,A^\ast]$. This is just the composition of $\mu_d$ with the projection from $\mathfrak{su}(d)^\ast$ to the dual of the Lie algebra of the subgroup $DSU(d) \leq SU(d)$ of diagonal elements of $SU(d)$, so it's the moment map of the conjugation action of $DSU(d)$ on $\Cd$.
%
% It looks to me like the $i$th entry of $\delta(A)$ is just $\|A_i\|^2 - \|A^i\|^2$, where $A_i$ is the $i$th row of $A$ and $A^i$ is the $i$th column. So if we think of $A$ as the adjacency matrix of a weighted digraph, then $\delta^{-1}(0)$ consists of those weighted digraphs for which the indegree equals the outdegree at every vertex, which are called flow networks or balanced weighted digraphs or something. (If you really want this indegree/outdegree interpretation, I guess you have to be a little careful and not let $A$ be the adjacency matrix, exactly, but let it be the matrix with entries given by the square roots of the weights on the graph.)
%
% So then I guess we more or less immediately get:
% \begin{enumerate}
%     \item The collection of complex flow networks (say with fixed total degree) is connected. This is presumably not new, because the constraints are linear constraints, so this is probably just the intersection of a linear subspace with a sphere.
%     \item You can take any arbitrary weighted digraph and flow it by the negative gradient flow of $\delta$ to get a valid flow network; importantly this will keep the weights real if they started out as real. Also, if the diagonal entries of $A$ are zero (which they presumably would be in flow applications), they will stay zero under this flow (which is \textit{not} true for flowing by $-\nabla\energy$); this is presumably another important feature.
% \end{enumerate}
% \#2 sounds like the sort of thing that might be interesting for certain applications. I guess one worry is that there's no particular reason to assume the gradient flow preserves positivity, so something weird may happen if entries become negative \textbf{Update:} In fact, the gradient flow \textit{does} preserve positivity, so this isn't an issue. Argument to come.
%
% \clay{Starting to write down some facts:}
% \begin{enumerate}
% 	\item I believe that
% 	\[
% 		\nabla \delta(A) = \left(4a_{ij}((\|A_i\|^2 - \|A^i\|^2)-(\|A_j\|^2-\|A^j\|^2))\right)_{i,j} = -4 [A,\diag([A,A^\ast])].
% 	\]
% 	So it looks to me like the critical points must satisfy $\|A_i\|^2-\|A^i\|^2=\|A_j\|^2-\|A^j\|^2$ for all $i$ and $j$. In other words, $\|A_i\|^2-\|A^i\|^2$ is independent of $i$. But $\sum_i \left(\|A_i\|^2-\|A^i\|^2\right) = \sum_i \|A_i\|^2 - \sum_i \|A^i\|^2 = \|A\|^2 - \|A\|^2=0$, so the only way $\|A_i\|^2-\|A^i\|^2$ can be independent of $i$ is if it is always 0. So the only critical points of $\delta$ are the global minima.
%
% 	\item If $A$ and $B$ are as in \Cref{rem:convexity}, then $\delta(A) = 0 = \delta(B)$, but $\delta((1-t)A+tB) = \energy((1-t)A+tB)=32t^2(1-t^2)>0$, so $\delta$ is invex but not quasiconvex.
%
% 	\item $\nabla\delta(A) = 4 \left. \frac{d}{d\epsilon}\right|_{\epsilon=0}\diag([A,A^\ast]) \cdot A$, so $\nabla \delta(A)$ is tangent to the $S((\C^\times)^d)$-orbit of $A$. In particular, the gradient flow preserves the spectrum. It also preserves the diagonal entries of $A$ since the diagonal of $\nabla \delta(A)$ is zero (more generally, it preserves all the principal minors, for whatever that's worth). In particular, then, this means that if the diagonal entries started at zero (for example, in the adjacency matrix of a weighted digraph), they will always stay zero (in graph terms, we don't spawn any spurious loop edges).
%
% 	\item Notice also that, in our formula for $\nabla \delta(A)$, if any $a_{ij}$ becomes 0, then the corresponding entry in $\nabla \delta(A)$ is also zero. So if gradient flow ever takes an entry to 0, it will get stuck there. In particular, this means that gradient flow cannot change the sign of an entry, so we don't have to worry about flowing to some weird negative weight. This also means that if $A$ starts with a zero in some entry, it will stay zero forever; in graph terms, this means that the gradient flow doesn't introduce any new edges.
%
% 	\item The negative gradient flow of $\delta$ does cause $\|A\|^2$ to go down. In terms of graphs, this means that some of the weight on the edges disappears from the system, which seems undesirable, so once again it is probably a good idea to flow within $\mathcal{U}_d$. If we let $\overline{\delta}$ be the restriction of $\delta$ to $\mathcal{U}_d$, then I believe that the intrinsic Riemannian gradient is
% 	\[
% 		\grad \overline{\delta}(A) = -4([A,\diag([A,A^\ast])]+\overline{\delta}(A)A).
% 	\]
% 	Notice that if some $a_{ij} = 0$, then the corresponding entry in $\grad \overline{\delta}(A)$ is also zero, so gradient flow will keep zeros where they are and preserve signs of entries in $A$.
%
% 	\item It looks to me like the same proof as in \Cref{lem:gradient dot product} shows that $\langle -\grad \overline{\delta}(A), \grad s(A) \rangle = 8 s(A) \overline{\delta}(A)$, so then the argument in \Cref{prop:non-nilpotency} will show that the negative gradient flow of $\overline{\delta}$ preserves non-nilpotency.
%
% 	\item If $A$ is a non-minimizing critical point, then $A = -\frac{1}{\overline{\delta}(A)}[A,\diag([A,A^\ast])]$ is of the form $A = [A,B]$, so the same Jacobson's Lemma argument as in \Cref{prop:critical points} will show that the non-minimizing critical points of $\overline{\delta}$ must be nilpotent.
%
% 	\item Putting the last two points together seems to prove that non-nilpotent matrices in $\mathcal{U}_d$ flow to balanced matrices in $\mathcal{U}_d$.
%
% 	\item A (weighted) directed graph is acyclic if and only if its adjacency matrix is nilpotent.\footnote{Here's a quick proof: the entries in $A^k$ count paths of length $k$. Suppose the graph has $n$ vertices. If it is acyclic, then any path has $\leq n-1$ edges (otherwise a vertex would repeat), so $A^n = 0$. If it is not acyclic, then there are paths of arbitrary length, because you can just keep going around a cycle, so every $A^k$ has at least one nonzero entry.} This fits with the above, since there's no way to balance a DAG without just sending all the edge weights to 0.
%
% \end{enumerate}

% \section{Examples and Applications}

% To do\dots

% \section{Random Notes on Literature, Etc.}

% \cite{noschese2009structured} consider the distance of a Toeplitz matrix to the variety of normal matrices.

% \cite{guglielmi2019computing} considers the problem of computing the closest normal matrix to a given matrix, particularly under constraints (real matrix must go to real normal matrix, fixed sparsity pattern). 

% \cite{ruhe1987closest} and \cite{gabriel1987normal} give algorithms for computing the closest normal matrix to a given matrix.

% References for balancing digraphs:

% \cite{rikos2014distributed} - Concerned with the ``distributed" problem. Here, we start with a graph (unweighted) and want to allow each node to control the weight of each outgoing edge. This is an iterative process; at each iteration, a given node knows how much flow is coming and going out, and is allowed to adjust the weights of its outgoing edges. The goal is for the process to converge to a weighted digraph.  Question: in gradient descent, what does the gradient update look like at each node? I.e., does the update take any non-local data into account? Answer: doing the calculations explicitly on a 3x3 matrix, this doesn't look to be the case.

% \cite{hooi1970class} - This is an old paper on the topic, motivated by traffic flow. The distributed aspect is not considered here, but the paper only considers integer weights. This constraint seems fairly common. The results are mostly theoretical. An algorithm for balancing a digraph is given, where one finds all circuits starting and ending at a given vertex. If all edges appear at least once, a weighting is then obtained by assigning weights based on the multiplicity with which each edge appears. Otherwise, all circuits are listed for another vertex, etc. This doesn't seem practical.

% \cite{hadjicostis2012distributed} - Considers the centralized (i.e., non-distributed) problem, as well as the distributed one. The centeralized algorithm requires a strongly connected graph (there is a directed path between any two nodes). The idea is as follows. If the graph is unbalanced, find a positively unbalanced and a negatively unbalanced node, find a path between them, increase all weights along the path by the negative unbalanced amount (in the paper it says to do it by the positively unbalanced amount, but this seems weird - need to double-check). Do this iteratively, and convergence is achieved after finitely many steps (they bound the required number). 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
